Like an Open Book? Read Neural Network Architecture with Simple Power Analysis on 32-bit Microcontrollers

Model extraction is a growing concern for the security of AI systems. For deep neural network models, the architecture is the most important information an adversary aims to recover. Being a sequence of repeated computation blocks, neural network models deployed on edge-devices will generate distinctive side-channel leakages. The latter can be exploited to extract critical information when targeted platforms are physically accessible. By combining theoretical knowledge about deep learning practices and analysis of a widespread implementation library (ARM CMSIS-NN), our purpose is to answer this critical question: how far can we extract architecture information by simply examining an EM side-channel trace? For the first time, we propose an extraction methodology for traditional MLP and CNN models running on a high-end 32-bit microcontroller (Cortex-M7) that relies only on simple pattern recognition analysis. Despite few challenging cases, we claim that, contrary to parameters extraction, the complexity of the attack is relatively low and we highlight the urgent need for practicable protections that could fit the strong memory and latency requirements of such platforms.

==> img/diagram_archi/display_archi_diagram_old.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[width=0.6\textwidth]{./img/diagram_archi/mnist_MLP_archi.png}
    \caption{MLP (MNIST)}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[width=0.85\textwidth]{./img/diagram_archi/mnist_CNN_archi.png}
    \caption{CNN (MNIST)}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{./img/diagram_archi/cifar10_CNN_archi.png}
    \caption{CNN (Cifar10)}
\end{subfigure}

\begin{subfigure}[t]{\textwidth}
\centering
\includegraphics[width=\textwidth]{./img/diagram_archi/test.PNG}
\caption{CNN (Cifar-10), simple version}
    
\end{subfigure}

\caption{Detailed architecture of considered models. \textcolor{red}{Objectif: le moins de texte inutile possible. "Volume shape" ça ne sert à rien. Simplifier au maximum en faisant une légende pour les 3 modèle. Exemple avec CNN Cifar-10}. NB: à l'impression les Output layer n'ont pas la même couleur}
\label{diagram_models_archi}
\end{figure}

==> img/traces/dense_AF_all.tex <==
%\begin{minipage}
\begin{figure}[h!]
\centering
\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/mnist_dense0.png}
    \caption{$1^{st}$ dense \textit{$N=23$ $\Leftrightarrow 5+3$ patterns}}
    \label{23_neur_MLP}
\end{subfigure}

\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/mnist_dense1.png}
    \caption{$2^{nd}$ dense \\\textit{ $N=18$ $\Leftrightarrow 4+2$ patterns}}
    \label{18_neur_MLP}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/mnist_dense2.png}
    \caption{$3^{rd}$ dense \\\textit{ $N=13$ $\Leftrightarrow 3+1$ patterns}}
    \label{13_neur_MLP}
\end{subfigure}

\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/mnist_framed_dense1.png}
    \caption{$2^{nd}$ dense \textbf{with triggers}\\\textit{ $N=18$ $\Leftrightarrow 4+2$ patterns}}
    \label{framed_18_neur_MLP}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/mnist_framed_dense2.png}
    \caption{$3^{rd}$ dense \textbf{with triggers}\\\textit{ $N=13$ $\Leftrightarrow 3+1$ patterns}}
    \label{framed_13_neur_MLP}
\end{subfigure}

\caption{EM activity overview of dense layers for the custom SP-MLP model. Expected patterns clearly appear for the first layer, not for the $2^{nd}$ and $3^{rd}$ %\simon{Est ce que le t=0 de la figure b correspond à t=0 de la figure d ? Si non, il faut ajouter qq chose qui le même en evidence. Par exemple, retrouver dans la fig d les barres verticales pointillé de la fig b. (idem pour c et e).} \textcolor{red}{effectivement: pourquoi on est 20 us plus court alors qu'on ajoute des triggers ?}
}
\label{trace_number_neurons_sp}

%\end{figure}
%\begin{figure}[!htb]
%\centering

\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./tab/af_duration.pdf}
    \vspace*{0.2mm}
    \caption{Layer duration according to used activation function}
    \label{tab:AF_duration}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/activation_functions/ReLU/zoom_trace_relu1.png}
    \caption{$2^{nd}$ ReLU layer}% - $924.25 \µs$}
    \label{ReLU_AF_1}
\end{subfigure}

\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/activation_functions/Sigmoid/zoom_trace_sigmoid1.png}
    \caption{$2^{nd}$ Sigmoid layer}% - $3.21 ms$}
    \label{Sigmoid_AF_1}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[h]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/activation_functions/Tanh/zoom_trace_tanh1.png}
    \caption{$2^{nd}$ Tanh layer}% - $3.58 ms$}
    \label{Tanh_AF_1}
\end{subfigure}

\caption{Zoom over the beginning of second activation layers with their duration}
\label{AF_patterns}
\end{figure}

%\end{minipage}


==> img/traces/dense_layer/special_cases/display_dense_special_cases.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/trace_dense0.png}
    \caption{$1^{st}$ dense layer of SP. dedicated MLP \textit{- 23 neur. $\Leftrightarrow 5+3$ patterns}}
    \label{23_neur_MLP}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/trace_dense1.png}
    \caption{$2^{nd}$ dense layer of SP. dedicated MLP \textit{- 18 neur. $\Leftrightarrow 4+2$ patterns}}
    \label{18_neur_MLP}
\end{subfigure}

\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/trace_dense2.png}
    \caption{$3^{rd}$ dense layer of SP. dedicated MLP \textit{- 13 neur. $\Leftrightarrow 3+1$ patterns}}
    \label{13_neur_MLP}
\end{subfigure}

\caption{EM activity overview of dense layers with special number of neurons}
\label{trace_number_neurons_sp}
\end{figure}

==> img/traces/dense_layer/special_cases/display_rect_traces.tex <==
\begin{figure}[!b]
\centering
\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/rect_trace_dense1.png}
    \caption{$2^{nd}$ dense layer of SP. dedicated MLP with triggers \textit{- 18 neur. $\Leftrightarrow 4+2$ patterns}}
\end{subfigure}\hspace{\fill}
\begin{subfigure}[t]{0.49\textwidth}
    \includegraphics[width=1\textwidth]{./img/traces/dense_layer/special_cases/rect_trace_dense2.png}
    \caption{$3^{rd}$ dense layer of SP. dedicated MLP with triggers \textit{- 13 neur. $\Leftrightarrow 3+1$ patterns}}
\end{subfigure}

\caption{EM activity of dense layers with trigger framing to be seen pattern}
\label{trace_number_neurons_sp_rect}
\end{figure}

==> src/experimental_results/exp_intro.tex <==
\begin{comment}
\subsection{Structure of Experimental Results} 
Each of the following section cover a specific kind of layer and are organised similarly. Firstly, details about process and results of the aforementioned layers are introduced and usually represented with listing. Then, method for recovering parameter value is described and illustrated with several traces corresponding to different use-cases. Finally, limitations of proposed method are discussed.
Three models are considered throughout following sections corresponding to different sizes and cases. Two of these three models are trained on MNIST dataset\cite{deng2012mnist}, a MLP and a CNN. Last models is a larger CNN trained with Cifar-10 colored images\cite{krizhevsky2009learning}. Models' detailed architecture is illustrated in diagram~\ref{diagram_models_archi}. Their accuracy over their test-set are respectively $95.8\%$, $98.0\%$ and $67.8\%$.
\end{comment}

\subsection{Models and datasets} 
Classically, we use two traditional benchmarks MNIST\footnote{\url{http://yann.lecun.com/exdb/mnist/}} (28x28 grayscale images, 10 labels) and Cifar-10\footnote{\url{https://www.cs.toronto.edu/~kriz/cifar.html}} (32x32 color images, 10 labels). For MNIST, we trained a MLP and a CNN with the TensorFlow platform that achieved respectively $95.8\%$ and $98.0\%$ on the test set. For Cifar-10, we trained a more complex CNN that reached $67.8\%$ on the test set. The architecture of these models are illustrated in Fig.~\ref{diagram_models_archi} (colors are used to identify the layer). 


\input{img/diagram_archi/display_archi_diagram}

\subsection{Target device and setup}}
Chosen experimental platform is a ARM Cortex-M7 based STM32H7 board. This high-end board is able to to embed state-of-the-art models (e.g., 8-bit quantized MobileNet for image classification task) thanks to its large memories (2 MBytes of flash memory and 1 MByte of RAM). A 25 MHz quartz has been melted as part of the HSE oscillator to have more stable clock. CPU is running at 25 MHz as well, as its clock is directly derived from the melted quartz.
Langer probe (EMV-Technik LF-U 2,5 with a frequency range going from 100 kHz to 50 MHz) is used to measure EM emanations coming from the unopened chip and is connected to a 200 MHz amplifier (Fento HVA-200M-40-F) with a 40 dB gain. Acquisitions are collected and saved thanks to a Lecroy WavePro 604HD-MS oscilloscope.


\subsection{Threat model}
The attacker aims to recover the architecture of an unknown quantized victim model with as much detail as possible. Table~\ref{tab:info_to_extra} lists all the information the adversary aims to extract thanks to a EM trace. 

The adversary is aware of the usage of CMSIS-NN module and has appropriate expertise in Deep Learning including the most classical and logical layer sequences. 
The adversary is able to acquire EM side-channel information leaking from the board while model inference is performed without limitation and without perturbing it (only usual behavior is considered). %Several traces can be obtained with several inference recorded for subsequent averaging. 
As explained in section~\ref{scope}, our goal is to evaluate how much information can be extracted in a minimal setting. Therefore, we consider that the attacker has only access to a single averaged EM trace corresponding to the inference of a single test input (not used in the training test).   %only one input, unseen during training phase, can be used by the attacker. Such input value isn't modified with chosen noise and tends to match targeted model's task.

\input{tab/information_to_extract}


\begin{comment}
\subsection{List of covered parameters}
As mentioned before, this work doesn't aim at being exhaustive and dealing with every type of layer available with NNoM and CMSIS-NN. Treated information about model's architecture are detailed below.

\begin{multicols}{2}
\begin{enumerate}
    \item Entire inference
    \begin{itemize}
        \item Number and type of layer
    \end{itemize}
    \item Convolution layers
    \begin{itemize}
        \item Output shape
        \item Number of kernels
        \item Size of kernels
        \item Deduced stride and padding
    \end{itemize}
    \item MaxPool layers
    \begin{itemize}
        \item Output shape
        \item Deduced filter size
    \end{itemize}
    \item Dense layers
    \begin{itemize}
        \item Number of neurons
    \end{itemize}
    \item Activation functions
    \begin{itemize}
        \item ReLU or not ReLU
    \end{itemize}
\end{enumerate}
\end{multicols}
\end{comment}


==> src/experimental_results/layer_number_and_nature.tex <==

%\subsection{Preliminary knowledge}
At first, an adversary may exploit the nature of the task performed by the model. In some case, it can give hints about the type of the victim model. Typically, a model performing a computer vision task is likely to be built around CNN principle. However, there is no strict rule that matches a task to a model type. Therefore, we claim that the knowledge of the task may provide a set of possible layer types that must be confirmed by a first analysis on the overall structure of the trace. Moreover, preliminary knowledge also encompasses the classical deep learning practices, more especially the \textit{logical} order of layers. It's typically relevant for CNN: if the first layer is identified as a convolutional one, a standard association is another conv. layer or a pooling one. 

The adversarial strategy follows a coarse-to-fine approach. The first information to extract is the overall structure of $\mathcal{A}_M$ with two information: the number of layers, $L$ and their natures. Then, the attacker focuses on each layer one after the other and, according to their nature, extracts a set of hyper-parameters easing to design a substitute model $M'_{\Theta}$. %that are compulsory to design a substitute model $M'_{\Theta}$.

\paragraph{Step 1: Finding the number of layers.}
When analyzing the general shape of the averaged EM trace, the very first observation is that it can be straightforwardly split into several blocks by identifying the boundaries that separate them. This can be made easier with a classical frequency spectrum that highlights the separation between the blocks, as illustrated in Fig.~\ref{cifar10_CNN_inf_spectro} for the Cifar-10 CNN. For the 3 models studied in this work, this simple analysis gives the exact number $L$ of layers for each model architecture $\mathcal{A}_M$. Figures \ref{trace_entire_inf} illustrate the identified  blocks for three models with the same colors as in Fig.~\ref{diagram_models_archi}. To validate that layers truly correspond to blocks, and for illustration purpose only, triggers have been added to clearly mark out layer boundaries. 

\paragraph{Step 2: Identifying layers' nature.}
According to their nature and input dimensions, layers will have different complexities which impact execution duration. The complexity of layers can be estimated in different ways. Here we classically consider the number of Multiplications and Accumulations (MACs). Such metric directly stems from computation to be effected and input dimensions, complexity of convolution and dense layers are respectively computed as follow:
\begin{equation}
    MAC_{Conv2D} = (Z^2 \times C_{in}) \times (H_{out}^2 \times C_{out})\text{, } MAC_{dense} = H_{in} \times H_{out}
\label{complex_mac}
\end{equation}
Complexity of the first layer of both MNIST models are $(3^2 \times 1) \times (28^2 \times 16) = 112896$ MACs for the CNN and $784 \times 32 = 25088$ MACs for the MLP. This complexity has direct repercussions in layer execution duration. Thus, usually, conv. layer would take longer to execute than dense one when having similar inputs. Other types of layers such as MaxPool and activation ones have a much reduced complexity due to the computation they perform.

\input{img/traces/entire_inference/display_entire_inf_and_nb_of_layers}

%In addition to this timing analysis
In addition to these temporal clues, the attacker can mostly leverage on specific EM activities related to each layer type (discussed in section~\ref{exp_section}) by considering smaller timescales. Thus, layer nature can be identified before doing more detailed analysis about their proper hyper-parameters.  
Once the first layer is identified, ML expertise and usual layers sequence knowledge can provide additional hints about next layers nature.  
This encourages the attacker to extract $\mathcal{A}_M$ by analysing model layers consecutively. With this general method along those dedicated to specific layers, DNN model architecture can be accurately recovered from an EM trace with a single input. 

==> tab/af_duration.tex <==

\begin{table}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc}
Layer & ReLU      & Sigmoid $(\tfrac{1}{ReLU})$ & Tanh $(\tfrac{1}{ReLU})$\\
\midrule
0     & 1.84ms    & 8.24ms  $(\times 4.5)$  & 8.24ms  $(\times 4.5)$ \\
1     & 0.92ms    & 3.21ms  $(\times 3.5)$  & 3.58ms  $(\times 3.9)$ \\
2     & 7.60µs    & 15.60µs $(\times 2)$    & 20.64µs $(\times 2.7)$ 
\end{tabular}%
%}
\caption{Layer duration according to used activation function}
\label{tab:AF_duration}
\end{table}



==> tab/algo_conv.tex <==
\begin{minipage}[t!]{0.46\linewidth}
\begin{algorithm}[H]\scriptsize
\caption{\texttt{fast} conv.}
\label{alg_conv_output_size_fast}
\begin{algorithmic}

% Top part
\State
\For{$\textcolor{red}{i_y \gets 0,\ i_y < P},\ i_y+1$}
\State \textit{/* Iterate over $H_{out}$ value */}
\For{$i_x \gets 0,\ i_x < H_{out},\ i_x+1$}
\State $im2col\_and\_GeMM()$ 
\EndFor
\EndFor

% Middle part
\State
\For{$\textcolor{red}{;,\ i_y < H_{out}-P},\ i_y+1$}
% Left part
\For{$i_x \gets 0,\ i_x < P,\ i_x+1$}
\State $im2col\_and\_GeMM()$
\EndFor
% Middle part
%\State\pam{Si P=0, ça revient à faire la boucle deux fois ???}
\For{$;,\ i_x < H_{out}-P,\ i_x+1$}
\State $im2col\_and\_GeMM()$
\EndFor
% Right part
\State
\For{$;,\ i_x < H_{out},\ i_x+1$}
\State $im2col\_and\_GeMM()$
\EndFor
\EndFor

% Bottom part
\State
\For{$\textcolor{red}{;,\ i_y < H_{out}},\ i_y+1$}
\For{$i_x \gets 0,\ i_x < H_{out},\ i_x+1$}
\State $im2col\_and\_GeMM()$
\EndFor
\EndFor
\State
\State $compute\_left\_over\_if\_any()$

\end{algorithmic}
\end{algorithm}

\end{minipage}
\hfill
\begin{minipage}[t!]{0.46\linewidth}

\begin{algorithm}[H]\scriptsize
\caption{\texttt{RGB} and \texttt{basic} conv.}\label{alg_conv_output_size_basic}
\begin{algorithmic}
\State \textit{/* Iterate over $H_{out}$ value */}
\For{$i_y \gets 0,\ \textcolor{red}{i_y < H_{out},\ i_y+1}$}
\State \textit{/* Here as well */}
\For{$i_x \gets 0,\ i_x < H_{out},\ i_x+1$}
\State $im2col\_and\_GeMM()$
\EndFor
\State $compute\_left\_over\_if\_any()$
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]\scriptsize
\caption{Matrix-product for conv. (\textbf{GeMM})}
\label{alg_conv_nb_kernel}
\begin{algorithmic}
\State $\textcolor{red}{rowCnt \gets C_{out} >> 1}$
\State \textit{/* Iterate over \#kernel/2 */}
\While{$\textcolor{red}{rowCnt}$}
\State $init\_sum\_with\_bias()$
\State $\textcolor{red}{colCnt \gets (C_{in} \times Z^2) >> 2}$
\While{$\textcolor{red}{colCnt}$}
\State $accumulate\_over\_vector()$
\State $colCnt \gets colCnt-1$
\EndWhile
\State $rowCnt \gets rowCnt-1$
\EndWhile
\State $compute\_left\_over\_if\_any()$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\\

==> tab/algo_gemm.tex <==
\begin{algorithm}[H]\scriptsize
\caption{Matrix-product for conv. (\textbf{GeMM})}
\label{alg_conv_nb_kernel}
\begin{algorithmic}
\State $\textcolor{red}{rowCnt \gets C_{out} >> 1}$
\State \textit{/* Iterate over \#kernel/2 */}
\While{$\textcolor{red}{rowCnt}$}
\State $init\_sum\_with\_bias()$
\State $\textcolor{red}{colCnt \gets (C_{in} \times Z^2) >> 2}$
\While{$\textcolor{red}{colCnt}$}
\State $accumulate\_over\_vector()$
\State $colCnt \gets colCnt-1$
\EndWhile
\State $rowCnt \gets rowCnt-1$
\EndWhile
\State $compute\_left\_over\_if\_any()$
\end{algorithmic}
\end{algorithm}

==> tab/algo_maxpool_dense.tex <==
\begin{minipage}[t!]{0.46\linewidth}
    
\begin{algorithm}[H]\scriptsize
\caption{MaxPool}\label{alg_maxpool}
\begin{algorithmic}
\State \textit{/* Pooling along x axis */}
\For{$i_y \gets 0,\ i_y < H_{in},\ i_y+1$}
\For{$i_x \gets 0,\ i_x < H_{out},\ i_x+1$} 
\State $define\_window\_start\_stop()$
\State $compare\_and\_remplace\_if\_larger()$
\EndFor
\EndFor
\State \textit{/* Pooling along y axis */}
\State $\textcolor{teal}{trigger\_up()}$
\State \textit{/* Directly iterate over $H_{out}$ */}
\For{$i_y \gets 0,\ \textcolor{red}{i_y < H_{out},\ i_y+1}$}
\State $define\_window\_start\_stop()$
\State $compare\_and\_remplace\_if\_larger()$
\EndFor
\State $\textcolor{teal}{trigger\_down()}$
\end{algorithmic}
\end{algorithm}

\end{minipage}
\hfill
\begin{minipage}[h]{0.46\linewidth}
    
\begin{algorithm}[H]\scriptsize
\caption{Dense layer}\label{alg_dense}
\begin{algorithmic}
\State $init()$
\State \textit{/* Nb. neurons divided by 4 */}
\State $\textcolor{red}{rowCnt \gets N >> 2}$
\While{$rowCnt$}
\State $init\_sums\_with\_bias()$
\State $colCnt \gets H_{in} >> 2$
\While{$colCnt$}
\State $increment\_weighted\_sums()$
\State $colCnt \gets colCnt-1$
\EndWhile
\State \textit{/* Get remainder of div. by 4 */}
\State $colCnt \gets H_{in} \& 0x3$
\While{$colCnt$}
\State $manage\_column\_left\_over()$
\State $colCnt \gets colCnt-1$
\EndWhile
\State $rowCnt \gets rowCnt-1$
\EndWhile
\State $\textcolor{red}{rowCnt \gets N \& 0x3}$
\While{$\textcolor{red}{rowCnt}$}
\State \textit{/* Manage remaining neurons */}
\State $manage\_row\_left\_over()$
\State $rowCnt \gets rowCnt-1$
\EndWhile
\end{algorithmic}
\end{algorithm}
    
\end{minipage}


==> tab/cmsis_conv_functions.tex <==

\begin{table}[]
\caption{CMSIS-NN convolution functions corresponding to observed traces}
\label{tab:cmsis_conv_functions}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|c|c}
\multicolumn{2}{l|}{Considered conv. layer} &
  Corresponding used CMSIS-NN function &
  Reasons \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mnist\\ CNN\end{tabular}} &
  $1^{st}$ conv. layer &
  \lstinline{arm\_convolve\_HWC\_q7\_basic()} &
  \begin{tabular}[c]{@{}c@{}}Squared shape and  single \\ input channel (gray scale picture)\end{tabular} \\
 &
  $2^{nd}$ conv. layer &
  \lstinline{arm\_convolve\_HWC\_q7\_fast()} &
  \begin{tabular}[c]{@{}c@{}}squared shape (\textgreater{}1),\\ input channel multiple of 4 \\ and output channel multiple of 2\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Cifar10\\ CNN\end{tabular}} &
  $1^{st}$ conv. layer &
  \lstinline{arm\_convolve\_HWC\_q7\_RGB()} &
  \begin{tabular}[c]{@{}c@{}}Squared shape and\\ 3 input channels (RGB)\end{tabular} \\
 &
  $2^{nd}$ conv. layer &
  \lstinline{arm\_convolve\_HWC\_q7\_fast()} &
  \begin{tabular}[c]{@{}c@{}}Squared shape (\textgreater{}1),\\ input channel multiple of 4\\ and output channel multiple of 2\end{tabular} \\
 &
  $3^{rd}$ conv.layer &
  \lstinline{arm\_convole\_HWC\_q7\_fast()} &
  \begin{tabular}[c]{@{}c@{}}Squared shape (\textgreater{}1),\\ input channel multiple of 4\\ and output channel multiple of 2\end{tabular}
\end{tabular}%
}
\end{table}

==> tab/cmsis_conv_functions_in_models.tex <==
\begin{table}[th]
\captionsetup{justification=justified}
\caption{CMSIS-NN convolution functions corresponding to observed traces}
\label{tab:cmsis_conv_functions_on_models}
\centering
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{llr}
\toprule
\multicolumn{2}{l}
{
\begin{tabular}[l]{@{}l@{}}Conv. layer number
\end{tabular}
} & 
\begin{tabular}[r]{@{}c@{}}Corresponding CMSIS-NN function
\end{tabular} \\ 

\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Mnist CNN\end{tabular}}   & 1 & \texttt{arm\_convolve\_HWC\_q7\_basic()}\\

 & 2 & \texttt{arm\_convolve\_HWC\_q7\_fast()} \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Cifar-10  CNN\end{tabular}} & 1 & \texttt{arm\_convolve\_HWC\_q7\_RGB()}  \\

& 2 & \texttt{arm\_convolve\_HWC\_q7\_fast()} \\

& 3 & \texttt{arm\_convolve\_HWC\_q7\_fast()} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tab/cmsis_conv_functions_requirements.tex <==
\begin{table}[]
\captionsetup{justification=justified}
\caption{CMSIS-NN convolution function requirements}
\label{tab:cmsis_conv_functions_req}
\centering
\begin{tabular}{c|c}
\begin{tabular}[c]{@{}c@{}}Corresponding\\ CMSIS-NN function\end{tabular} & Requirements                                                                                             \\ \hline
\lstinline{arm\_convolve\_HWC\_q7\_basic()} & \begin{tabular}[c]{@{}c@{}}Squared shape and single\\ input channel (gray scale picture)\end{tabular}                                  \\
\lstinline{arm\_convolve\_HWC\_q7\_RGB()}   & \begin{tabular}[c]{@{}c@{}}Squared shape and\\ 3 input channels (RGB)\end{tabular}                                                     \\
\lstinline{arm\_convolve\_HWC\_q7\_fast()}  & \begin{tabular}[c]{@{}c@{}}Squared shape (\textgreater{}1),\\ input channel multiple of 4and output channel multiple of 2\end{tabular}
\end{tabular}
\end{table}

==> tab/conv_output_dim_sumup.tex <==
\begin{table}[H]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Mnist}     & \multicolumn{2}{c}{Cifar-10}  \\
\midrule
Layer                & $H_{out}$     & $N_{p}$ & $H_{out}$     & $N_{p}$ \\
1                    & 28            & 392           & 32            & 512           \\
2                    & 14            & 98            & 16            & 128           \\
3                    & $\varnothing$ & $\varnothing$ & 8             & 32\\
\bottomrule

\end{tabular}
%}
\caption{Conv. layer output dimension \\and theoretic number of pattern}
\label{tab:Conv_out_dim}
\end{table}

==> tab/global_overview.tex <==

\begin{table}[h!]
    \centering
    \caption{Overview of recovered parameters, related prerequisites and extraction method. \textit{Italic elements} stem from threat model}
    \includegraphics[width=1\textwidth]{tab/tableau_recap_contrib.pdf}
    \label{tab:param_overview}
\end{table}




==> tab/xtr_method.tex <==
\begin{table}[h!]
\centering
\caption{Architecture extraction method overview. \textit{elements} stem from threat model, \textit{P.}: Pattern, \textit{I/O}: Input/Output}
\label{tab:xtr_method}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc}
\hline
Target &
  hyper-parameter &
  Prerequisites &
  Method outlines &
  Limitations \\ \hline
\multirow{4}{*}{Conv} &
  $H_{out}$ &
  \begin{tabular}[c]{@{}c@{}}CMSIS loop\\ handling\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Count \#\textit{P.}\\ then compute\end{tabular} &
  Possibly high \#\textit{P.} \\
  \cmidrule{2-5}
 &
  $K$ &
  CMSIS factor 2 &
  Count \#\textit{P.} &
  None \\
  \cmidrule{2-5}
 &
  $Z$ &
  \begin{tabular}[c]{@{}c@{}}\# input channels,\\ CMSIS factor 4\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Count \#\textit{P.}\\ then compute\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Possibly low \#\textit{P.} \&\\ hard to distinguish\end{tabular} \\
  \cmidrule{2-5}
 &
  $S, P$ &
  \textit{I/O} shape, $Z$ &
  \begin{tabular}[c]{@{}c@{}}Inequality\\ computation\end{tabular} &
  Requires $Z$ \\ \hline
\multirow{2}{*}{MaxPool} &
  $H_{out}$ &
  None &
  Count \#\textit{P.} &
  None \\
  \cmidrule{2-5}
 &
  $Z_{pool}$ &
  \textit{I/O} shape &
  Compute &
  None \\ \hline
Dense &
  $N$ &
  CMSIS factor 4 &
  Count \#\textit{P.} &
  \begin{tabular}[c]{@{}c@{}}\textit{P.} can be hard\\ to distinguish,\\ Special cases when\\ \#neurons $\% 4 \neq 0$\end{tabular} \\ \hline
AF &
  ReLU or not &
  \begin{tabular}[c]{@{}c@{}}ReLU\\ function \textit{P.}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textit{P.} Id.,\\ Layer delay\end{tabular} &
  Only distinguish ReLU \\ \hline
%\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Entire\\ inference\end{tabular}} &
\multirow{2}{*}{$\mathcal{A}_M$} &
  \# layers &
  \textit{Model task} &
  \begin{tabular}[c]{@{}c@{}}Id. blocks,\\ Spectrograms\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Sequence of dense layers\\ with reduced size can be\\ hard to distinguish\end{tabular} \\
  \cmidrule{2-5}
 &
  \begin{tabular}[c]{@{}c@{}}Nature of\\ layers\end{tabular} &
  \textit{\begin{tabular}[c]{@{}c@{}}Model task,\\ ML expertise,\\ Input tensor shape\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Id. first layer,\\ Id. blocks \textit{P.}\\ \& duration\end{tabular} &
  None
\end{tabular}%
}
\end{table}
